X-Former: In-Memory Acceleration of Transformers

Transformers have achieved great success in a wide variety of natural language processing (NLP) tasks due to the attention mechanism, which assigns an importance score for every word relative to other words in a sequence. However, these models are very large, often reaching hundreds of billions of parameters, and therefore require a large number of DRAM accesses. Hence, traditional deep neural network (DNN) accelerators such as GPUs and TPUs face limitations in processing Transformers efficiently. In-memory accelerators based on non-volatile memory promise to be an effective solution to this challenge, since they provide high storage density while performing massively parallel matrix vector multiplications within memory arrays. However, attention score computations, which are frequently used in Transformers (unlike CNNs and RNNs), require matrix vector multiplications (MVM) where both operands change dynamically for each input. As a result, conventional NVM-based accelerators incur high write latency and write energy when used for Transformers, and further suffer from the low endurance of most NVM technologies. To address these challenges, we present X-Former, a hybrid in-memory hardware accelerator that consists of both NVM and CMOS processing elements to execute transformer workloads efficiently. To improve the hardware utilization of X-Former, we also propose a sequence blocking dataflow, which overlaps the computations of the two processing elements and reduces execution time. Across several benchmarks, we show that X-Former achieves upto 85x and 7.5x improvements in latency and energy over a NVIDIA GeForce GTX 1060 GPU and upto 10.7x and 4.6x improvements in latency and energy over a state-of-the-art in-memory NVM accelerator.

==> sections/subsections/speedup_techniques.tex <==
{\noindent} As mentioned earlier, the generation of the non-ideal conductance matrices is very slow and, while acceptable for inference (where it is one-time), does scale to DNN training (where it needs to be invoked after each minibatch, when weights change). 
%Since DNN training changes weights (upon update) after each minibatch iterations, causing scaling difficult even after using optimized BLAS routines.
Therefore, we present two complementary speedup techniques that significantly accelerate training simulation while preserving good modeling fidelity.


%------------------------------------------------------------------------
\begin{figure}[htb]
	\vspace*{-10pt}
    \centering
    \includegraphics[width=\columnwidth]{img/norderapprox.jpg}
 	\vspace*{-6pt}
    \caption{(a) Approximate Analytical Model overview, (b) Accuracy comparison for various crossbar array models} 
    \label{fig:approx}
	\vspace*{-6pt}
\end{figure}
%------------------------------------------------------------------------

\noindent\textbf{Approximate analytical model (AAM).} The current at the output column in a non-ideal crossbar can be viewed as a sum of many terms, each corresponding to a path through the crossbar. In the AAM model, we consider a subset of these paths (typically the shorter paths from each row to each column), while ignoring the longer paths (as shown in Figure~\ref{fig:approx}(a)). The current for each path is computed considering the source ($r_{source}$), sink ($r_{sense}$), and wire resistances ($r_{row}$ and $r_{col}$). The AAM model allows us to seamlessly trade-off efficiency for accuracy by simply considering more or fewer paths.

We plot the modeling error of AAM with respect to FCM for 64x64 crossbars with different $R_{min}$-$R_{max}$ ranges in Figure~\ref{fig:error}. As shown, AAM is not suitable for case(c) with low $R_{min}$-$R_{max}$ as it results in considerable errors. However, for higher $R_{min}$-$R_{max}$ range [case (a)] modeling errors are negligible, and in case (b), modeling errors are quite small. Therefore, AAM is used selectively only when the synaptic device resistance range is much higher than wire resistances.


%------------------------------------------------------------------------
\begin{figure}[htb]
	\vspace*{-6pt}
    \centering
    \includegraphics[width=\columnwidth]{img/errorMap.jpg}
	\vspace*{-14pt}
    \caption{Error-map of Approximate Analytical model w.r.t FCM for different resistance ranges}
    \label{fig:error}
	\vspace*{-6pt}
\end{figure}
%------------------------------------------------------------------------

\noindent\textbf{Interpolated-FCM}. In this speedup technique, we perform FCM selectively -- only once every L minibatch iterations (as opposed to each iteration). Every time FCM is performed, the net synaptic conductance distortion due to non-idealities (($G_{ideal}$-$G_{non-ideal}$)/$G_{ideal}$) is profiled and stored. For the subsequent L-1 iterations, the $G_{non-ideal}$ is computed using the stored distortion profile. Figure~\ref{fig:approx}(b) shows the application-level accuracy for various models --FCM, AAM, and Interpolated-FCM for the LetNet-5 DNN on MNIST dataset. As shown, the speedup techniques can effectively model DNN training without much loss in modeling fidelity (note the highly magnified y-axis range).


%----------------------------------------------------------------------
% \begin{comment}
%
% %\vspace*{-10pt}
% \begin{algorithm}
% \caption{Algorithm for nth interval FCM}
% \label{alg:ninterval}
% \begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \renewcommand{\algorithmicrepeat}{\textbf{Begin}}
% \renewcommand{\algorithmicuntil}{\textbf{End}}
% \renewcommand{\algorithmiccomment}[1]{\hfill// \textit{#1}}
% \REQUIRE{Pixels of the training images} 
% \ENSURE {Trained Network considering all the nonidealities}
% \STATE {Begin}
% %\STATE {$DNN_{FxP}$ = $DNN_{FP}$ // $DNN_{FxP}$: Fixed-Point DNN }
% %\FOR {Each layer k: 1 to N}
% %\STATE{[$WD_{k}$, $AD_{k}$]=get-magnitude-distribution ($DNN_{FxP}$, ValData)}
% %\STATE{[$WST_{list}$, $AST_{list}$]= get-saturationPts ($WD_{k}$, $AD_{k}$, pW, pA)}
% %\STATE{$Acc_{list}$ = getDNNaccuracy ($DNN_{FxP}$,$WST_{list}$, $AST_{list}$,ValData)
% %\STATE{[$wst_{opt}$, $ast_{opt}$]} = getOptConversion ($DNN_{FxP}$,$WD_{k}$, $AD_{k}$, pW, pA,ValData)
% %\STATE { $DNN_{FxP}$ = convertToFxP ($DNN_{FxP}$,[$wst_{opt}$, $ast_{opt}$], k)}
% %\ENDFOR
% \STATE {All the training hyper parameters are initialized;} 
% %\STATE { [$\alpha_{g}$, $\beta_{g}$] = get-Conversion-Params ($g_{max}$, $g_{min}$, pW) }
% \STATE {count=0;}
% \FOR {epochnumber: 1 to the total\_epochs}
% \FOR {batchno: 1 to total\_batches}
% \IF{batchno $\%$ interval == 0}
% \STATE{fcm();}
   % \STATE{ perc\_forward$=$new\_weights$/$old\_weights;}
  % \STATE{forward();}
 % \STATE{fcm();}
   % \STATE{perc\_backward$=$new\_weights$/$old\_weights;}
    % \STATE{backward();}
% \ELSE
  % \STATE {new\_weights$=$old\_weights*perc\_forward;}
  % \STATE{forward();}
    % \STATE{new\_weights$=$old\_weights*perc\_backward;}
   % \STATE{backward();}
% \ENDIF
% \STATE{update();}
% \ENDFOR
% \ENDFOR
% \STATE {Return Accuracy}
% %\STATE {End}
% \end{algorithmic}
% \end{algorithm}
% \vspace*{-10pt}
% \end{comment}
%
%------------------------------------------------------------------------



%The fast crossbar model (FCM) used in the non-ideal conductance transformer block is not scalable and takes lot of compute hours due to the numerous number of matrix inversions. Larger crossbar sizes increases the time taken to perform a single matrix inversion whereas more number of crossbar instances (smaller crossbar size) leads to higher number of times a matrix inversion is performed. The large number of parameters make it extremely difficult to scale the FCM operations in spite of using optimized blas routines. To that effect, we propose two speed up techniques in addition to the fast crossbar model which makes our model scalable and produce close to accurate results compared to that of the actual FCM model. This approximate schemes are based on the assumption that the device resistance is substantially larger than the wire parasitics. The accuracy results for a LeNet-5 architecture evaluated on the MNIST dataset is showed in Figure.\ref{fig:approx} to show the effectiveness of the two speedup schemes. We propose the following speedup techniques: 
